Perigee: Efficient Peer-to-Peer Network Design for Blockchains

A key performance metric in blockchains is the latency between when a transaction is broadcast and when it is confirmed (the so-called, confirmation latency). While improvements in consensus techniques can lead to lower confirmation latency, a fundamental lower bound on confirmation latency is the propagation latency of messages through the underlying peer-to-peer (p2p) network (inBitcoin, the propagation latency is several tens of seconds). The de facto p2p protocol used by Bitcoin and other blockchains is based on random connectivity: each node connects to a random subset of nodes. The induced p2p network topology can be highly suboptimal since it neglects geographical distance, differences in bandwidth, hash-power and computational abilities across peers. We present Perigee, a decentralized algorithm that automatically learns an efficient p2p topology tuned to the aforementioned network heterogeneities, purely based on peers' interactions with their neighbors. Motivated by the literature on the multi-armed bandit problem, Perigee optimally balances the tradeoff between retaining connections to known well-connected neighbors, and exploring new connections to previously-unseen neighbors. Experimental evaluations show that Perigee reduces the latency to broadcast by $33\%$. Lastly Perigee is simple, computationally lightweight, adversary-resistant, and compatible with the selfish interests of peers, making it an attractive p2p protocol for blockchains.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> properties.tex <==
\section{Discussion} \label{s:discussion}

\subsection{Preventing Eclipse Attacks}

The p2p layer of Bitcoin has been found to be particularly vulnerable to Eclipse attacks~\cite{saad2019exploring}, 
%, heilman2015eclipse, marcus2018low, nayak2016stubborn}, 
in which an adversary controlling a large number of IP addresses, forces a victim to form all connections to the adversarial nodes, thereby isolating it from the rest of the network. 
Bitcoin nodes maintain knowledge of other peers in the network, using \texttt{tried} and \texttt{new} address tables, which contain IP addresses of nodes previously connected to, and nodes never connected to before, respectively~\cite{heilman2015eclipse}. 
When a node restarts, it uses the addresses available in the tables---particular those added or updated recently---to form its connections. 
This particular way to forming connections enables an adversary to execute the Eclipse attack; therefore a recommended countermeasure is to select neighbors randomly regardless of when they were added to the \texttt{tried} or \texttt{new} tables. 
Such a countermeasure is naturally built into \namens.
The continuous random exploration of new candidate neighbors in \namens, in fact, offers a much stronger form of protection by not only connecting to nodes randomly upon restarts, but periodically doing so. 

% - also Sybil attacks 

% - incentive for forwarding blocks?? 
%- partitioning attack~\cite{tran2020stealthier}

\subsection{Protocol Incentives}

 Bitcoin today adopts mechanisms by which nodes disconnect from neighbors that willfully forward illegitimate transactions or blocks~\cite{nakamoto2019bitcoin}. 
However, there are currently no incentive mechanisms that prevent nodes from not  actively participating in the block relaying process. 
\name fills this crucial gap. 
With \namens, nodes have an incentive to relay blocks promptly to avoid being disconnected by their neighbors, and taking a hit in block reception times. % eventually becoming isolated. 

% -- leaching off of well connected servers is ok, but server should should only allocate a bounded amount of resources for incoming peers (e.g., constant number of connections) 
% - or forward blocks to neighbors in the order of their scores 

\begin{figure*}[!tbp]
  \centering
  \subfloat[]{\includegraphics[width=0.3\textwidth]{fig/FullyDeploy.png}\label{fig:FullyDeploy}}
  \centering
%  \subfloat[Histogram]{\includegraphics[width=0.51\textwidth, height = 9cm]{fig/histogram_link_latencies.png}\label{fig:f2}}
  \subfloat[]{\includegraphics[width=0.3\textwidth]{fig/PartialDeploy.png}\label{fig:PartialDeploy}}
    \centering
%  \subfloat[Histogram]{\includegraphics[width=0.51\textwidth, height = 9cm]{fig/histogram_link_latencies.png}\label{fig:f2}}
  \subfloat[]{\includegraphics[width=0.43\textwidth]{fig/DistributionDifferenceBetweenThem.png}\label{fig:DistributionDifferenceBetweenThem}}
  \caption{Propagation delays under partial deployment of \namens. (a) 100\% of nodes follow \namens-Subset. (b) Only 10\% of nodes follow \namens, while the remaining 90\% of nodes are randomly connected. (c) Performance of the nodes that follow \name (left), and those that do not (right).  
  % In Fig~\ref{fig:f1}, mean for UCB, vanilla scoring, subset scoring, random and geographical algorithms are $48.10$, $54.58$, $59.42$, $180.24$ and $165.44$ respectively. Median is $30$, $10$, $20$, $168.5$ and $146$, respectively. $90$ percentile is $120$, $180$, $160$, $334.5$ and $327$, respectively.
  }
  \label{fig:PartialDep}
\end{figure*}

\subsection{Partial Deployment}
In this section, we show that the network as a whole benefits even if only a small number of nodes follow \namens. 
Figure~\ref{fig:PartialDep} shows a simulation in which only 10\% of the nodes follow \namens-Subset while the remaining 90\% of the nodes choose their neighbors randomly. 
% In reality, it's hard for all the nodes to follow the same neighbor selection strategy, what if there are some nodes refusing our algorithm or only partial node accept?
% Based on our simulation on \name Subset at Section 5.3, we run a simulation with only 10\% nodes to follow the \name Subset algorithm while the other 90\% nodes keep the original random selection.
For comparison, Figure~\ref{fig:FullyDeploy} shows the performance when all 100\% of the nodes follow \namens. 
Under partial deployment, while the network fails to achieve the same level of performance as with full deployment, there does seem to be significant gain in latencies for both nodes following \name and those that do not (Figure~\ref{fig:PartialDeploy}). 
% In Figure~\ref{fig:PartialDeployment}, the partial deployment fails to reach the same delay due to the remaining uncooperative nodes.
The nodes that deploy \name see a slighly better latency as shown in Figure~\ref{fig:DistributionDifferenceBetweenThem}.
% However, in column c, the nodes that deploy our algorithm can have a much advantage to the other nodes.
% Our algorithms can do help to decrease the delay to the network with exploiting and exploring, the neighbor selection can help to optimize the connection whether the other nodes follow or nor. 



%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.47\textwidth]{fig/PartialDeployment.png}
%    \caption{Delay distribution for partial deployment} 
%    \label{fig:PartialDeployment}
%\end{figure}














==> related.tex <==
\section{Related Work} \label{s:related}

The problem of speeding up block propagation has received considerable attention in the blockchain community: for example using block compression \cite{}. There are also cryptographic and coding techniques to reduce the message overhead in block forwarding. 
For example, in Graphene a combination of Bloom filters and IBLTs are used to compact the messages needed for syncing the local copies of blockchain across the \pp network. In Velocity~\cite{chawla2019velocity},  on the other hand, fountain codes are used for decentralized delivery of blocks and subsequent reconstruction at the peer.


However, optimizing the \pp topology itself for faster delivery in blockchains has not received as much attention. While much work has been done in traditional 
% Constructing overlays with small diameter is a well-studied topic in the \pp literature~\cite{pandurangan2003building}.
An exception is Kadcast~\cite{rohrer2019kadcast} which proposes using the Kademlia's structured overlay, and UDP-based block forwarding, for  
% on the underlying P$2$P network layer in blockchain networks have explored using a structured P$2$P overlay for 
a more efficient propagation. 
Many structured overlays for efficient content storage and lookup, including with good locality properties~\cite{rowstron2001pastry}, have been proposed in the past but they are not explicitly optimized for broadcast traffic~\cite{lua2005survey}. 
Indeed Bitcoin, and other popular blockchains, do not require communication primitives beyond simple broadcasting of messages, and this is a key reason why an unstructured random topology has sufficed there. For example, the Bitcoin p2p network does not support sending messages targeted to a particular peer (unicast).
% , in Kadcast, a peer is oblivious to link bandwidth, link latencies, node latencies etc., while filling the buckets under bucket eviction policy. 
% In terms of network latency, this renders the performance of eventual underlying P$2$P network equivalent to that of random algorithm. 
% One way to take latency into account is to look at geography of node based on it's IP ~\cite{kaune2008embracing, abboud2009underlay}. 
% However, an adversarial peer can spoof geo-location using VPN or proxy. 
% In contrast, \name does not need to know anything about neighbors and thus, is robust to geolocation spoofing.

Some prior work for blockchains has focused on building dedicated high-speed low-latency distribution networks, such as bloXroute~\cite{klarman2018bloxroute}, Falcon, FIBRE. 
% Another line of work is fast relay networks, which includes bloXroute~\cite{bloxroute}, Falcon, FIBRE. 
These solutions are not fully decentralized as using them requires the peers to place trust on the distribution network in the middle. 
The routes are also susceptible to man-in-the-middle attack. 
% Nevertheless, even if such relay networks are present in the blockchain ecosystem, \name automatically adapts to the existence of such distribution networks. 
% Another line of work has focused on using cryptographic and coding techniques to reduce the message overhead in block forwarding. 
% For example, in Graphene a combination of Bloom filters and IBLTs are used to compact the messages needed for syncing the local copies of blockchain across the \pp network.
% Orthogonal to our work is the recently proposed Graphene~\cite{ozisik2017graphene} and Velocity protocols~\cite{chawla2019velocity} that focus on reducing the message overhead. 
% In Graphene, a combination of Bloom filters and IBLTs are used to compact the messages needed for syncing the local copies of blockchain across the P$2$P network. 



